TropeTwist: Trope-based Narrative Structure Generation

Games are complex, multi-faceted systems that share common elements and underlying narratives, such as the conflict between a hero and a big bad enemy or pursuing a goal that requires overcoming challenges. However, identifying and describing these elements together is non-trivial as they might differ in certain properties and how players might encounter the narratives. Likewise, generating narratives also pose difficulties when encoding, interpreting, and evaluating them. To address this, we present TropeTwist, a trope-based system that can describe narrative structures in games in a more abstract and generic level, allowing the definition of games' narrative structures and their generation using interconnected tropes, called narrative graphs. To demonstrate the system, we represent the narrative structure of three different games. We use MAP-Elites to generate and evaluate novel quality-diverse narrative graphs encoded as graph grammars, using these three hand-made narrative structures as targets. Both hand-made and generated narrative graphs are evaluated based on their coherence and interestingness, which are improved through evolution.

==> tables/table1.tex <==
\begin{table*}[t!]
    \begin{tabularx}{\textwidth}{s|sb}

  Name                     & Symbol   & Definition                                                                                            \\ \hline
Hero &
  HERO &
  A protagonist character that is usually imbued with pure good qualities, such as rightness, friendship, well-rounded skill set, and superior moral. In a team lineup, the hero stands front and center. \\
Five-man band            & 5MA      & A specific type of hero group composed by up-to-five characters whose members fall into archetypes which all complement one another. \\
The chosen one &
  NEO &
  A specific type of hero that has been chosen by some force and becomes the only one capable of resolving the plot. \\
Superhero &
  SH &
  A specific type of hero with unique abilities, frequently costumed to keep a secret identity. \\
Conflict                 & CON & A non-specific problem to overcome that drives a story and links to other story elements.             \\
% Conflict against nature  & CONA     & A specific type of conflict that comes from natural sources.                                          \\
% Conflict against society & COSO     & A specific type of conflict that originates in the social environment.                                \\
Enemy                    & ENEMY    & A nemesis to the hero in that it opposes to her and her qualities.                                    \\
Empire &
  EMP &
  A specific type of collective enemy that resembles historical empires that ambition conquering the world in which the story takes place. \\
Big bad                  & BAD      & A specific type of enemy that impersonates the ultimate cause for all the bad events in a story.      \\
Dragon                   & DRA      & A specific type of enemy that acts as the right hand of the big bad.                                  \\
Plot device                 & PLD & A feature or element that drives the plot forward.                                                          \\
Chekhov's gun            & CHK      & A plot device that qualifies a story element as relevant to the story or a conflict.                     \\
MacGuffin                & MCG      & A plot device that makes a story driven by an element whose nature is irrelevant.               \\
May help you in your quest                         & MHQ      & A plot device that denotes a story element as important to resolve a conflict.                                                                                   
\end{tabularx}
\caption{Tropes included thus far in Story Designer depicted by their name, symbol, and definition, extracted from \cite{tvtropes}.}
\label{tab:tropes}
\end{table*}

==> tables/table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[t]
\caption{Tropes included and used in TropeTwist, extracted from~\cite{tvtropes}.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|l}
Name                       & \textit{Symbol} & \textit{Definition}                                                                  \\ \hline
Hero                       & HERO            & A protagonist character.                                                             \\
Five-man band              & 5MA             & Hero group composed by up-to-five archetypical characters                            \\
The chosen one             & NEO             & Specific hero chosen as the one.                                                     \\
Superhero                  & SH              & Specific hero with unique abilities.                                                 \\
Conflict                   & CONF             & Non-specific problem to overcome between characters.                                 \\
Enemy                      & ENEMY           & A nemesis to the hero.                                                               \\
Empire                     & EMP             & Collective enemy with the ambition of conquering the world.                          \\
Big bad                    & BAD             & Specific enemy, which is the ultimate cause for all the bad.                         \\
Dragon                     & DRAKE             & Specific enemy, which is the right hand of BAD.                                      \\
Plot device                & PLD             & A feature or element that drives the plot forward.                                   \\
Chekhov's gun              & CHK             & A plot device that qualifies a story element as relevant to the story or a conflict. \\
MacGuffin                  & MCG             & A plot device that makes a story driven by an element whose nature is irrelevant.    \\
May help you in your quest & MHQ             & A plot device that denotes a story element as important to resolve a conflict.      
\end{tabular}%
}
\label{tab:tropes}
\end{table*}

%  thus far in Story Designer depicted by their name, symbol, and definition, extracted from \cite{tvtropes}.
